CoFRIDA: Self-Supervised Fine-Tuning for Human-Robot Co-Painting

Prior robot painting and drawing work, such as FRIDA, has focused on decreasing the sim-to-real gap and expanding input modalities for users, but the interaction with these systems generally exists only in the input stages. To support interactive, human-robot collaborative painting, we introduce the Collaborative FRIDA (CoFRIDA) robot painting framework, which can co-paint by modifying and engaging with content already painted by a human collaborator. To improve text-image alignment, FRIDA's major weakness, our system uses pre-trained text-to-image models; however, pre-trained models in the context of real-world co-painting do not perform well because they (1) do not understand the constraints and abilities of the robot and (2) cannot perform co-painting without making unrealistic edits to the canvas and overwriting content. We propose a self-supervised fine-tuning procedure that can tackle both issues, allowing the use of pre-trained state-of-the-art text-image alignment models with robots to enable co-painting in the physical world. Our open-source approach, CoFRIDA, creates paintings and drawings that match the input text prompt more clearly than FRIDA, both from a blank canvas and one with human created work. More generally, our fine-tuning procedure successfully encodes the robot's constraints and abilities into a foundation model, showcasing promising results as an effective method for reducing sim-to-real gaps.

==> figures_text/fig_3_failed_simulation.tex <==
% \begin{figure}
%     \centering \small
%     \includesvg[width=\columnwidth]{figures/co_creative_mistakes.svg}
%     \caption{
%     The FRIDA painting simulation fails to accurately reproduce source images for a number of reasons leading to a Semantic Sim2Real Gap: (a) different or (b) more colors in the source than available to the robot, (c) the source cannot be represented with the limited available strokes the robot can make, and (d) the fine details in the source cannot be represented with the size of the brush available to the robot.}
%     \label{fig:co_creative_mismatch}
% \end{figure}

==> unused.tex <==

% In the case of drawing and painting, co-creation is often done by human artists taking turns adding and modifying the contents of a piece~\cite{codrawingsSeattle2020,jansen2021coDrawWorkflows}.
% Co-creation's major benefit comes in the realm of shared autonomy whereby a user needs to feel like they are autonomous and contributing to the overall piece rather than handing over all of the task to the robot~\cite{selvaggio2021autonomy, bretan2016-roboticDrummer}. 
% Co-creation as a mechanism also supports the dynamic aspects of Art whereby the goal of a piece may and should evolve throughout the process~\cite{hertzmann2022algorithmicPainting}.
% \cite{herath2020artsHealth} installed a robot that draws in a hospital to investigate its abilities to affect the health of the people staying and working their. The robot was not interactive, but participants strongly agreed that the robot reduced their anxiety, was enjoyable, improved their day, and made them feel more positive. No participant disagreed that they would consider using robots as therapeutic tools in the future.
% \cite{davis2016DrawingApprentice} found that a collaborative drawing agent could augment the creativity of an artist on a computer based interface.
% \cite{bateman2021creating} interviewed 16 animators at various stages in careers and found that a collaborative tool would be preferable to a tool that automates whole aspects of their work.
% \cite{lin2020cobbie} found that their robot, Cobbie, as opposed to a virtual agent produced sketches with higher perceived novelty, 
%     Two potential reasons for this was the slowness of the real robot and the noisy performance of the robot due to real-world stochasticity.
%     People enjoyed playing and interfering with the robot as it drew.
%     Participants considered the robot a partner and the virtual agent a tool.
%     Participants expressed interest in future design iterations that would include multi-modal inputs including language and more detailed sketches from the robot.
%     Participants found the robot more friendly than the agent.


% \begin{figure*}[h]
%     \centering \small
%     \includesvg[width=0.7\textwidth]{figures/inpainting.svg}
%     \caption{[I will make major revisions to this if it makes it in the paper] In-painting is not a solution because (1) we want to be able to make global edits, and (2) we want the created content to engage with the existing content, not zero it out and replace. I think the top result looks pretty good, inpainting picks up on the style and even when you add back the original strokes it doesn't mess up the content too much. The bottom example doesn't engage with the existing content well.}
%     \label{fig:inpainting}
% \end{figure*}

% s opposed to virtual agents which perform text-to-image, our robot needs to perform text-and-canvas-to-image and needs to be able to plan robot actions to create the desired image. To train a model to do the action prediction directly would take on the order of hundreds of millions of training examples, as this is what it took to train state-of-the-art text-to-image models~\cite{rombach2021stableDiffusion, ramesh2021dallE}. There is also a paradox, text-action pairs are needed to train the painting model but to get these implies the existence of a robot that can paint from text already.  An alternative to training a feed-forward model would be to do synthesis through optimization using a pre-trained text-image encoder~\cite{jain2023vectorfusion, schaldenbrand2022styleclipdraw, frans2021-clipdraw, schaldenbrand2023frida}, however, this gradient descent planning results in noisy images that loosely resemble the desired text content.

